Models in the Loop: Aiding Crowdworkers with Generative Annotation Assistants

In Dynamic Adversarial Data Collection (DADC), human annotators are tasked with finding examples that models struggle to predict correctly. Models trained on DADC-collected training data have been shown to be more robust in adversarial and out-of-domain settings, and are considerably harder for humans to fool. However, DADC is more time-consuming than traditional data collection and thus more costly per annotated example. In this work, we examine whether we can maintain the advantages of DADC, without incurring the additional cost. To that end, we introduce Generative Annotation Assistants (GAAs), generator-in-the-loop models that provide real-time suggestions that annotators can either approve, modify, or reject entirely. We collect training datasets in twenty experimental settings and perform a detailed analysis of this approach for the task of extractive question answering (QA) for both standard and adversarial data collection. We demonstrate that GAAs provide significant efficiency benefits with over a 30% annotation speed-up, while leading to over a 5x improvement in model fooling rates. In addition, we find that using GAA-assisted training data leads to higher downstream model performance on a variety of question answering tasks over adversarial data collection.

==> Generative Annotation Assistants - NAACL2022/tables/as_aos.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{6.4pt}
\begin{tabular}{llrrr}
    \textbf{Model} & \textbf{Training Data} & \textbf{SQuAD\textsubscript{dev}} & \textbf{AddSent} & \textbf{AddOneSent}\\
    \midrule
    
    \multirow{2}{*}{BERT\textsubscript{Large}} & SQuAD & 90.3 & 73.7 & 80.3 \\
    & SQuAD + AdversarialQA & \textbf{93.3} & \textbf{80.1} & \textbf{85.2} \\
    
    \midrule
    
    \multirow{4}{*}{RoBERTa\textsubscript{Large}} & SQuAD & 93.5 & 82.4 & 86.9 \\
    & SQuAD + AdversarialQA & 92.5 & 83.4 & 86.7 \\
    & SQuAD + AdversarialQA + SynQA & 94.8 & 86.0 & 89.0 \\
    & SQuAD + AdversarialQA + SynQA\textsubscript{Ext} & \textbf{94.9} & \textbf{87.1} & \textbf{90.1} \\
    
    \midrule
    
    \multirow{3}{*}{ELECTRA\textsubscript{Large}} & SQuAD & 94.4 & 85.0 & 89.0 \\
    & SQuAD + AdversarialQA & 94.7 & \textbf{86.1} & \textbf{89.9} \\
    & SQuAD + AdversarialQA + SynQA & \textbf{94.8} & 85.7 & 89.2 \\
    
    \bottomrule
\end{tabular}
\caption{
%
Word-overlap \fone{} results for BERT, RoBERTa, and ELECTRA on the \squadone{} dev set and the AddSent and AddOneSent adversarial evaluation sets~\cite{jia2017adversarial}.
%
}
\label{tab:results_addsent}
\end{table*}

==> Generative Annotation Assistants - NAACL2022/tables/qs_per_example.tex <==
\begin{table}
\centering
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\begin{tabular}{ l c c }
    \multirow{2}{*}{\textbf{Feature}} & \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{7.9em}{\textbf{Avg. \#Generations per Example}}
    \\
    \\
    
    \midrule
    
    \multirow{3}{*}{GAA Training} & SQuAD & 0.69 \\
    & AdversarialQA & 0.86 \\
    & Combined & 0.83 \\
    
    \midrule
    
    \multirow{3}{*}{Sampling} & \textit{Likelihood} & 0.67 \\
    & \textit{Adversarial} & 0.87 \\
    & \textit{Uncertainty} & 0.83 \\
    
    \midrule

    \multirow{2}{*}{Answer Prompt?} & \crossmark{} & 0.73 \\
    & \checkmark{} & 0.91 \\
    
    \bottomrule
\end{tabular}
\caption{
%
Results showing how often annotators query the GAA for different experimental settings.
%
}
\label{tab:qs_per_example}
\end{table}

==> Generative Annotation Assistants - NAACL2022/tables/results_answer_prompting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.4pt}
        \begin{tabular} {@{\extracolsep{0pt}} p{0.14\textwidth} p{0.11\textwidth} | c c c | c c c c | c @{}}
                \textbf{GAA Training} &
                \textbf{Sampling} &
                
                \textbf{t (s)} & 
                \textbf{vMER (\%)} & 
                \textbf{t/vMFE (s)} & 
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule

            % Exp ID 15
            AdversarialQA & \textit{Likelihood} & \textbf{38.5}\std{22.7} & 5.63 & 988          & 83.8 & 49.7 & \textbf{40.3} & \textbf{30.7} & 55.9 \\
            % Exp ID 17
            AdversarialQA & \textit{Adversarial} & 44.2\std{21.6} & 9.46 & \textbf{668} & 83.9 & 48.7 & 36.2 & 30.3 & 55.2 \\
            % Exp ID 19
            AdversarialQA & \textit{Uncertainty} & 49.9\std{24.8} & 7.80 & 854         & 84.8 & \textbf{51.3} & 38.9 & 30.6 & 56.3 \\
            
        \midrule
        
            % Exp ID 14
            Combined & \textit{Likelihood} & 45.9\std{23.4} & 2.90 & 2,196               & \textbf{85.2} & 51.1 & 37.5 & 28.1 & \textbf{56.4} \\
            % Exp ID 16
            Combined & \textit{Adversarial} & 56.3\std{27.1} & \textbf{9.53} & 785              & 83.5 & 48.4 & 35.5 & 29.3 & 55.5 \\
            % Exp ID 18
            Combined & \textit{Uncertainty} & 57.6\std{27.7} & 4.48 & 1,841              & 83.4 & 47.4 & 36.6 & 27.8 & 55.2 \\
            
        \bottomrule
        \end{tabular}
    \caption{
    %
    Results for the investigation into supporting adversarial data collection using GAAs equipped with answer prompting. We investigate two different GAA training dataset sources, and three sampling strategies. The adversarial QA model-in-the-loop is identical for all settings.
    %
    }
    \label{tab:results_answer_prompting}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_baselines.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5.3pt}
        \begin{tabular} {@{\extracolsep{0pt}} c | c c c | c c c c | c @{}}
                \textbf{Adversary-in-the-loop?} & 
                
                \textbf{t (s)} & 
                \textbf{vMER (\%)} & 
                \textbf{t/vMFE (s)} & 
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule
            % Exp ID 0
            \crossmark & \textbf{57.2}\std{23.9} & 0.63 & 11,537 & \textbf{85.7} & 43.5 & 28.3 & 21.1 & 52.0 \\ 
            % Exp ID 4
            \checkmark & 61.5\std{27.1} & \textbf{1.86} & \textbf{4,863} & 85.0 & \textbf{53.0} & \textbf{34.2} & \textbf{26.9} & \textbf{58.8} \\
        \bottomrule
        \end{tabular}
    \caption{
    %
    Baseline results comparing standard and adversarial data collection. \textit{t} shows the median time taken per example in seconds and median absolute deviation (subscript). \textit{vMER} is the validated model error rate. \textit{t/vMFE} is the time per validated model-fooling example. Lower is better for the time-dependent metrics. Downstream evaluation is measured by training an ELECTRA\textsubscript{Large} QA model on the collected datasets and evaluating \fone{} scores on the \squadone{} dev set, the AdversarialQA test sets, and the MRQA dev sets for domain generalisation.
    %
    }
    \label{tab:results_baselines}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_improving_adversarial.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.4pt}
        \begin{tabular} {@{\extracolsep{0pt}} p{0.14\textwidth} p{0.11\textwidth} | c c c | c c c c | c @{}}
                \textbf{GAA Training} &
                \textbf{Sampling} &
                
                \textbf{t (s)} & 
                \textbf{vMER (\%)} & 
                \textbf{t/vMFE (s)} & 
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule

            % Exp ID 5
            \squad{} & \textit{Likelihood} & 61.1\std{31.9} & 2.25 & 3,501   & \textbf{86.5} & 50.1 & 30.1 & 24.1 & 57.6 \\
            % Exp ID 8
            \squad{} & \textit{Adversarial} & 62.6\std{22.7} & 4.66 & 1,750   & 83.2 & 48.1 & 27.7 & 24.2 & 55.0 \\
            % Exp ID 11
            \squad{} & \textit{Uncertainty} & 62.1\std{26.3} & 2.41 & 3,317   & 86.1 & \textbf{51.8} & 31.1 & 24.4 & \textbf{58.4} \\
            
        \midrule
        
            % Exp ID 6
            AdversarialQA & \textit{Likelihood} & 54.2\std{24.4} & 3.09 & 2,458   & 84.7 & 49.8 & 36.9 & \textbf{29.8} & 56.8 \\
            % Exp ID 9
            AdversarialQA & \textit{Adversarial} & 63.9\std{25.6} & \textbf{6.30} & \textbf{1,262}   & 83.3 & 49.4 & 34.9 & 28.1 & 56.7 \\
            % Exp ID 12
            AdversarialQA & \textit{Uncertainty} & 72.1\std{30.9} & 5.20 & 1,776   & 83.6 & 50.3 & \textbf{37.3} & 27.0 & 55.7 \\
            
        \midrule
        
            % Exp ID 7
            Combined & \textit{Likelihood} & \textbf{53.6}\std{25.6} & 2.64 & 2,724   & 85.1 & 48.9 & 33.4 & 24.7 & 56.5 \\
            % Exp ID 10
            Combined & \textit{Adversarial} & 69.6\std{29.6} & 4.86 & 1,922   & 82.9 & 48.0 & 33.6 & 28.6 & 54.5 \\
            % Exp ID 13
            Combined & \textit{Uncertainty} & 62.0\std{25.0} & 4.87 & 1,690   & 85.3 & 50.5 & 33.9 & 28.8 & 56.5 \\
            
        \bottomrule
        \end{tabular}
    \caption{
    %
    Results for the investigation into supporting adversarial data collection using GAAs. We investigate three different GAA training dataset sources, and three sampling strategies. The adversarial QA model used in the annotation loop is identical for all settings.
    %
    }
    \label{tab:results_improving_adversarial}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_improving_standard.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{4.4pt}
        \begin{tabular} {@{\extracolsep{0pt}} p{0.23\textwidth} | c c c | c c c c | c @{}}
                \textbf{Sampling Strategy} &
                
                \textbf{t (s)} & 
                \textbf{vMER (\%)} & 
                \textbf{t/vMFE (s)} & 
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule
            % Exp ID 1
            \textit{Likelihood} & \textbf{37.5}\std{21.4} & 0.62 & 8,708   & \textbf{85.5} & 41.8 & 25.3 & 20.3 & 53.6 \\ 
            % Exp ID 2
            \textit{Adversarial} & 55.6\std{20.9} & \textbf{4.02} & \textbf{1,760}  & 84.7 & \textbf{45.5} & 26.1 & 20.0 & \textbf{54.3} \\ 
            % Exp ID 3
            \textit{Uncertainty} & 63.1\std{28.6} & 2.77 & 3,018  & 83.2 & \textbf{45.5} & \textbf{28.2} & \textbf{21.9} & 53.2 \\ 

        \bottomrule
        \end{tabular}
    \caption{
    %
    Results for the investigation into supporting standard data collection using GAAs. Since this setting assumes no access to adversarially-sourced data, we use a generative model trained only on questions from \squadone{}. There is no adversarial QA model in the loop in this setting.
    %
    }
    \label{tab:results_improving_standard}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_mrqa.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=2pt
    \belowrulesep=2pt
    \renewcommand{\arraystretch}{1.5}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2pt}
        \begin{tabular} {@{\extracolsep{0pt}} p{0.19\textwidth} c | c c c c c c c c c c c c @{}}
                \multirow{2}{10em}{\textbf{GAA Details}} &
                \multirow{2}{2.3em}{\textbf{Adv?}} &
                \multicolumn{6}{c}{\textit{MRQA in-domain}} &
                \multicolumn{6}{c}{\textit{MRQA out-of-domain}} \\
                \hhline{~~||------||------}
                & &
                \scriptsize HotpotQA & 
                \scriptsize NQs & 
                \scriptsize NewsQA & 
                \scriptsize SearchQA & 
                \scriptsize \squad{} & 
                \scriptsize TriviaQA & 
                \scriptsize BioASQ & 
                \scriptsize DROP & 
                \scriptsize DuoRC & 
                \scriptsize RACE & 
                \scriptsize RelExt. & 
                \scriptsize TextbookQA \\
        
        \toprule

            % Exp ID 0
            - & \crossmark & 64.5 & 58.9 & 51.7 & 16.5 & 84.9 & 55.9 & 61.5 & 28.1 & 50.4 & 38.1 & 81.9 & 31.3 \\
            
            % Exp ID 4
            - & \checkmark & 65.3 & \textbf{65.4} & \textbf{57.2} & 36.6 & 85.0 & 62.2 & 66.9 & 43.4 & 55.5 & 44.1 & 83.4 & 41.1 \\
            
        \midrule
            
            % Exp ID 1
            \squad{} (\textit{Likelihood}) & \crossmark & 58.0 & 61.5 & 53.9 & 23.3 & 85.4 & 59.5 & 64.0 & 32.5 & 54.2 & 36.3 & 81.6 & 33.4 \\
            % Exp ID 2
            \squad{} (\textit{Adversarial}) & \crossmark & 56.7 & 63.8 & 55.4 & \textbf{37.4} & 84.1 & 55.4 & 60.7 & 30.4 & 53.9 & 38.8 & 75.5 & 39.3 \\
            % Exp ID 3
            \squad{} (\textit{Uncertainty}) & \crossmark & 62.3 & 62.0 & 53.5 & 26.3 & 83.4 & 57.6 & 63.0 & 30.9 & 50.5 & 37.0 & 79.6 & 32.2 \\
            
        \midrule
            % Exp ID 5
            \squad{} (\textit{Likelihood}) & \checkmark & \textbf{67.3} & 62.9 & 56.9 & 30.3 & \textbf{86.7} & 60.8 & 66.1 & 39.0 & 54.7 & 43.2 & 81.8 & 41.8 \\
            % Exp ID 8
            \squad{} (\textit{Adversarial}) & \checkmark & 60.5 & 61.6 & 51.4 & 30.8 & 83.3 & 59.7 & 62.5 & 38.1 & 52.7 & 39.9 & 80.7 & 39.5 \\
            % Exp ID 11
            \squad{} (\textit{Uncertainty}) & \checkmark & 62.7 & 65.3 & 55.9 & 32.9 & 86.3 & 63.8 & 65.2 & 40.4 & 56.4 & \textbf{44.4} & 81.3 & \textbf{46.0} \\
            
        \midrule
        
            % Exp ID 6
            AdvQA (\textit{Likelihood}) & \checkmark & 63.5 & 62.6 & 53.3 & 23.5 & 84.9 & 59.9 & 66.7 & \textbf{49.5} & 53.3 & 41.5 & 83.7 & 39.4 \\
            % Exp ID 9
            AdvQA (\textit{Adversarial}) & \checkmark & 60.8 & 63.2 & 52.9 & 33.2 & 83.8 & 59.5 & 63.9 & 44.8 & 53.4 & 40.8 & 81.4 & 43.2 \\
            % Exp ID 12
            AdvQA (\textit{Uncertainty}) & \checkmark & 62.3 & 61.8 & 53.3 & 26.0 & 83.6 & \textbf{64.0} & 62.5 & 47.6 & 52.9 & 39.4 & 81.8 & 32.9 \\
            
        \midrule
        
            % Exp ID 7
            Combined (\textit{Likelihood}) & \checkmark & 61.6 & 62.6 & 56.1 & 21.3 & 85.0 & 58.8 & \textbf{67.7} & 46.9 & \textbf{56.5} & 43.3 & 79.1 & 39.6 \\
            % Exp ID 10
            Combined (\textit{Adversarial}) & \checkmark & 60.8 & 60.4 & 51.8 & 30.0 & 82.7 & 55.7 & 61.2 & 42.6 & 53.5 & 38.5 & 79.6 & 37.4 \\
            % Exp ID 13
            Combined (\textit{Uncertainty}) & \checkmark & 64.7 & 64.2 & 53.5 & 27.3 & 85.4 & 59.1 & 64.4 & 45.5 & 49.2 & 41.1 & 83.5 & 40.6 \\
            
        \midrule
            & \multicolumn{12}{c}{\textit{Results below are for the settings with answer prompting}} \\
        \midrule
        
            % Exp ID 15
            AdvQA (\textit{Likelihood}) & \checkmark & 60.4 & 63.9 & 51.8 & 26.8 & 83.5 & 56.9 & 65.8 & 48.4 & 51.7 & 42.5 & 81.0 & 38.0 \\
            % Exp ID 17
            AdvQA (\textit{Adversarial}) & \checkmark & 60.0 & 63.8 & 51.3 & 25.0 & 83.7 & 60.4 & 65.0 & 48.6 & 49.9 & 40.4 & 83.3 & 31.0 \\
            % Exp ID 19
            AdvQA (\textit{Uncertainty}) & \checkmark & 62.7 & 64.0 & 51.2 & 32.9 & 84.9 & 58.3 & 66.3 & 47.0 & 45.4 & 42.3 & 83.0 & 37.9 \\
            
        \midrule
        
            % Exp ID 14
            Combined (\textit{Likelihood}) & \checkmark & 63.4 & 63.9 & 55.1 & 24.5 & 83.2 & 60.6 & 66.7 & 47.0 & 55.9 & 39.3 & 82.2 & 34.9 \\
            % Exp ID 16
            Combined (\textit{Adversarial}) & \checkmark & 62.0 & 63.7 & 51.6 & 18.2 & 83.5 & 60.6 & 64.6 & 48.5 & 53.4 & 40.4 & \textbf{83.8} & 35.3 \\
            % Exp ID 18
            Combined (\textit{Uncertainty}) & \checkmark & 60.6 & 62.9 & 54.2 & 25.0 & 83.6 & 59.2 & 63.3 & 44.4 & 52.5 & 41.6 & 80.3 & 35.3 \\
            
        \bottomrule
        \end{tabular}
    \caption{
    %
    Result breakdown for all twenty experiment modes on the MRQA evaluation sets.
    %
    }
    \label{tab:results_mrqa}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_plussquad_answer_prompting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{13.0pt}
        \begin{tabular} {@{\extracolsep{0pt}} p{0.14\textwidth} p{0.12\textwidth} | c c c c | c }
                \textbf{GAA Training} &
                \textbf{Sampling} &
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule

            % Exp ID 15
            AdversarialQA & \textit{Likelihood} & \textbf{89.2} & 53.9 & \textbf{43.4} & \textbf{31.9} & 59.7 \\
            % Exp ID 17
            AdversarialQA & \textit{Adversarial} & 89.1 & 53.4 & 36.4 & 28.0 & 58.8 \\
            % Exp ID 19
            AdversarialQA & \textit{Uncertainty} & 88.5 & \textbf{55.4} & 37.6 & 27.5 & 59.0 \\
            
        \midrule
        
            % Exp ID 14
            Combined & \textit{Likelihood} & \textbf{89.2} & 55.0 & 38.4 & 29.8 & \textbf{61.0} \\
            % Exp ID 16
            Combined & \textit{Adversarial} & 88.6 & 54.7 & 37.7 & 29.4 & 59.4 \\
            % Exp ID 18
            Combined & \textit{Uncertainty} & 88.8 & 53.1 & 32.6 & 26.7 & 57.5 \\
            
        \bottomrule
        \end{tabular}
    \caption{
    %
    Results for the investigation into supporting adversarial data collection using GAAs equipped with answer prompting when combining with 2k \squad{} training examples. We investigate two different GAA training dataset sources, and three sampling strategies. The adversarial QA model-in-the-loop is identical for all settings.
    %
    }
    \label{tab:results_plussquad_answer_prompting}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_plussquad_baselines.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{18.0pt}
        \begin{tabular} {@{\extracolsep{0pt}} c | c c c c | c }
                \textbf{Adversary-in-the-loop?} & 
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule
            % Exp ID 0
            \crossmark & 88.9 & 49.8 & 28.6 & 22.7 & 56.1 \\ 
            % Exp ID 4
            \checkmark & \textbf{89.3} & \textbf{53.2} & \textbf{34.1} & \textbf{27.3} & \textbf{60.1} \\
        \bottomrule
        \end{tabular}
    \caption{
    %
    Baseline results comparing standard and adversarial data collection. Downstream evaluation is measured by training an ELECTRA\textsubscript{Large} QA model on each of the collected datasets combined with 2k \squad{} training examples (for a total of 4k examples) and evaluating \fone{} scores on the \squadone{} dev set, the AdversarialQA test sets, and the MRQA dev sets for domain generalisation.
    %
    }
    \label{tab:results_plussquad_baselines}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_plussquad_improving_adversarial.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{13.0pt}
        \begin{tabular} {@{\extracolsep{0pt}} p{0.14\textwidth} p{0.12\textwidth} | c c c c | c}
                \textbf{GAA Training} &
                \textbf{Sampling} &
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule

            % Exp ID 5
            \squad{} & \textit{Likelihood} & 89.4 & 51.4 & 31.7 & 24.1 & 58.8 \\
            % Exp ID 8
            \squad{} & \textit{Adversarial} & 88.4 & 50.9 & 31.8 & 23.2 & 59.3 \\
            % Exp ID 11
            \squad{} & \textit{Uncertainty} & \textbf{89.6} & 53.8 & 31.6 & 25.3 & 59.0 \\
            
        \midrule
        
            % Exp ID 6
            AdversarialQA & \textit{Likelihood} & 89.3 & 52.4 & 38.1 & \textbf{30.2} & \textbf{60.6} \\
            % Exp ID 9
            AdversarialQA & \textit{Adversarial} & 88.8 & 54.0 & 34.5 & 27.0 & 59.3 \\
            % Exp ID 12
            AdversarialQA & \textit{Uncertainty} & 88.8 & 54.5 & \textbf{39.2} & 30.0 & 58.3 \\
            
        \midrule
        
            % Exp ID 7
            Combined & \textit{Likelihood} & 88.9 & \textbf{54.6} & 37.4 & 27.7 & 58.7 \\
            % Exp ID 10
            Combined & \textit{Adversarial} & 89.0 & 53.2 & 34.9 & 25.7 & 58.3 \\
            % Exp ID 13
            Combined & \textit{Uncertainty} & 88.9 & 54.4 & 35.9 & 26.9 & 57.8 \\
            
        \bottomrule
        \end{tabular}
    \caption{
    %
    Results for the investigation into supporting adversarial data collection using GAAs when combining with 2k \squad{} training examples. We investigate three different GAA training dataset sources, and three sampling strategies. The adversarial QA model used in the annotation loop is identical for all settings.
    %
    }
    \label{tab:results_plussquad_improving_adversarial}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Generative Annotation Assistants - NAACL2022/tables/results_plussquad_improving_standard.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \aboverulesep=0pt
    \belowrulesep=0pt
    \renewcommand{\arraystretch}{1.2}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{13.0pt}
        \begin{tabular} {@{\extracolsep{0pt}} p{0.32\textwidth} | c c c c | c }
                \textbf{Sampling Strategy} &
                
                \textbf{\squad{}\textsubscript{dev}} & 
                \textbf{\dataset{BiDAF}} & 
                \textbf{\dataset{BERT}} & 
                \textbf{\dataset{RoBERTa}} & 
                
                \textbf{MRQA} \\
        
        \toprule
            % Exp ID 1
            \textit{Likelihood} & \textbf{88.9} & 49.2 & 29.0 & 22.8 & 56.7 \\ 
            % Exp ID 2
            \textit{Adversarial} & 88.7 & \textbf{52.0} & \textbf{30.1} & \textbf{24.5} & \textbf{58.1} \\ 
            % Exp ID 3
            \textit{Uncertainty} & 88.5 & 50.0 & 29.7 & 22.8 & 57.1 \\ 

        \bottomrule
        \end{tabular}
    \caption{
    %
    Results for the investigation into supporting standard data collection using GAAs when combining with 2k \squad{} training examples. There is no adversarial QA model in the loop in this setting.
    %
    }
    \label{tab:results_plussquad_improving_standard}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
